WorkBenchMark: A LEGO-Based Assembly Benchmark with an Assembly-by-Disassembly Baseline for the Smart Manufacturing League

We introduceWorkBenchMark, a LEGO Duplo-based robotic assembly benchmark motivated by the RoboCup Smart Manufacturing League. Robotic assembly couples low-level manipulation with task-level symbolic reasoning under physical constraints, a combination that current end-to-end learning methods do not yet solve reliably. The benchmark provides 400 tasks across four complexity tiers. We provide an open-vocabulary perception, Assembly-by-Disassembly baseline solution. Our planning-based pipeline outperforms a modern vision-language-action approach across all tiers. The benchmark, simulation environment, and baseline implementation will be released openly to support the broader robotic assembly community.

==> acronyms.tex <==
\RequirePackage{acronym}

\acrodef{SML}{RoboCup Smart Manufacturing League}
\acrodef{ABD}{Assembly-by-Disassembly}
\acrodefindefinite{ABD}{an}{an}
\acrodefplural{ABD}{Assembly-by-Disassemblies}

==> admin.tex <==
\RequirePackage{mfirstuc}
% Highlighting & Editing Commands 
\newcommand{\showme}[1]{{\color{magenta} #1}}
\newcommand{\notes}[1]{{\color{cyan} #1}}
\newcommand{\revisit}[1]{{\color{blue} #1}}
\ifcomments
\newcommand{\added}[1]{{\color{red} #1}\xspace}
\newcommand{\altorig}[1]{{\color{brown} #1}\xspace}
\newcommand{\alt}[2]{\textcolor{green}{#1} $\backslash$ \textcolor{brown}{#2}\xspace}
\newcommand{\remove}[1]{{\color{green}\ #1}\xspace}
\newcommand{\removeifneeded}[1]{{\color{cyan} #1}\xspace}
\newcommand{\removehide}[1]{}
\newcommand{\addCRC}[1]{}
\else
\newcommand{\added}[1]{#1}
\newcommand{\altorig}[1]{}
\newcommand{\alt}[2]{#2}
\newcommand{\remove}[1]{}
\newcommand{\removeifneeded}[1]{}
\newcommand{\removehide}[1]{}
\newcommand{\addCRC}[1]{}
\fi

\newcommand{\altCRC}[2]{#1}

\ifcomments
\newcommand{\todocustom}[3]{\todo[linecolor=#2,backgroundcolor=#2!25,bordercolor=#2,#3]{#1}}
\else
\newcommand{\todocustom}[3]{}
\fi
\newcommand{\generalComment}[4][]{\todocustom{{\bf #3}: #4}{#2}{inline,size=\scriptsize,caption={},#1}}
\newcommand{\customtodo}[4][]{\generalComment[noinline,size=\scriptsize,#1]{#2}{TODO (#3)}{#4}}

\newcommand{\addauthor}[2]{%
  \expandafter\newcommand\csname color#1\endcsname{#2}%
  \expandafter\newcommand\csname todo#1\endcsname[2][]{%
    \customtodo[##1]{\csname color#1\endcsname}{\makefirstuc{#1}}{##2}%
  }%
  \expandafter\newcommand\csname comment#1\endcsname[2][]{%
    \generalComment[##1]{\csname color#1\endcsname}{\makefirstuc{#1}}{##2}%
  }%
}

